Online Fast Adaptation and Knowledge Accumulation: a New Approach to Continual Learning

Continual learning studies agents that learn from streams of tasks without forgetting previous ones while adapting to new ones. Two recent continual-learning scenarios have opened new avenues of research. In meta-continual learning, the model is pre-trained to minimize catastrophic forgetting of previous tasks. In continual-meta learning, the aim is to train agents for faster remembering of previous tasks through adaptation. In their original formulations, both methods have limitations. We stand on their shoulders to propose a more general scenario, OSAKA, where an agent must quickly solve new (out-of-distribution) tasks, while also requiring fast remembering. We show that current continual learning, meta-learning, meta-continual learning, and continual-meta learning techniques fail in this new scenario. We propose Continual-MAML, an online extension of the popular MAML algorithm as a strong baseline for this scenario. We empirically show that Continual-MAML is better suited to the new scenario than the aforementioned methodologies, as well as standard continual learning and meta-learning approaches.

==> neurips_2020.tex <==
% \documentclass{article}

% % if you need to pass options to natbib, use, e.g.:
%     \PassOptionsToPackage{numbers, compress}{natbib}
% % before loading neurips_2020

% % ready for submission
% \usepackage{neurips_2020}

% % to compile a preprint version, e.g., for submission to arXiv, add add the
% % [preprint] option:
%     % \usepackage[preprint]{neurips_2020}

% % to compile a camera-ready version, add the [final] option, e.g.:
%     % \usepackage[final]{neurips_2020}

% % to avoid loading the natbib package, add option nonatbib:
%     %  \usepackage[nonatbib]{neurips_2020}

% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage[colorlinks,linktoc=all]{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography

% %-------- Our packages ---------%
% % recommended, but optional
% %\usepackage{microtype}
% \usepackage{graphicx}
% % \usepackage{subfigure}
% \usepackage{booktabs} % for professional tables
% %
% \usepackage[usenames,dvipsnames]{xcolor}
% \usepackage[algo2e,ruled,linesnumbered,lined]{algorithm2e}
% \usepackage{amsmath}
% \usepackage{amsfonts}
% \newcommand{\mytodo}[1]{\textcolor{red}{#1}} 
% \newcommand{\new}[1]{\textcolor{blue}{#1}} 
% \usepackage{makecell}
% \usepackage{soul}
% \usepackage{wrapfig}
% \usepackage{caption}
% \usepackage{lipsum}
% \usepackage{subcaption}
% % \usepackage[colorinlistoftodos]{todonotes}
% \usepackage[colorinlistoftodos,disable]{todonotes}
% \usepackage{comment}



% % \usepackage{hyperref}
% \hypersetup{citecolor=BurntOrange}
% \hypersetup{linkcolor=MidnightBlue}
% \hypersetup{urlcolor=MidnightBlue}
% \usepackage[capitalise,nameinlink]{cleveref}
% \crefname{algorithm}{Alg.}{Algs.}
% \Crefname{algorithm}{Algorithm}{Algorithms}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \crefname{table}{Tab.}{Tabs.}
% \Crefname{table}{Table}{Tables}
% \crefname{appendix}{App.}{Apps.}
% \Crefname{appendix}{Appendix}{Appendixes}


% % Attempt to make hyperref and algorithmic work together better:
% \newcommand{\theHalgorithm}{\arabic{algorithm}}
% \newcommand{\std}[1]{ \color{darkgray}\tiny{$\pm$#1} }

% \renewcommand{\paragraph}[1]{{\bf #1}\;\;\;}

% % \renewcommand\thealgorithm{}
% % \newcommand{\setalglineno}[1]{%
% % \setcounter{ALC@line}{\numexpr#1-1}}

% %-------------------------------%


% %------ Variable --------%

% \newcommand{\newsetting}{Online faSt Adaptation and Knowledge Accumulation} 
% \newcommand{\newacron}{OSAKA} 

% % \newcommand{\firstFeature}{\textit{knowing what to train on}} 
% % \newcommand{\firstFeatureAcron}{KWTO} 

% \newcommand{\firstFeature}{update modulation}
% \newcommand{\FirstFeature}{Update modulation}
% \newcommand{\firstFeatureAcron}{UM} 

% \newcommand{\secondFeature}{prolonged adaptation phase} 
% \newcommand{\SecondFeature}{Prolonged adaptation phase} 
% \newcommand{\secondFeatureAcron}{PAP} 

% \def \rmSectionSpace {0.06cm}
% % \def \rmSubsectionSpace {0.05cm}
% % \def \rmSectionSpace {0.cm}
% \def \rmSubsectionSpace {0.02cm}
% \def \trimSize {0.0cm}

% %------------------------%

% %% two more lines if we change the title
% % \vspace{-\rmSectionSpace}
% \title{Online Fast Adaptation and Knowledge Accumulation (OSAKA): \\ a New Approach to Continual Learning}
% % \title{Online Fast Adaptation and Knowledge Accumulation}
% % \vspace{-\rmSectionSpace}

% % The \author macro works with any number of authors. There are two commands
% % used to separate the names and addresses of multiple authors: \And and \AND.
% %
% % Using \And between authors leaves it to LaTeX to determine where to break the
% % lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% % authors names on the first line, and the last on the second line, try using
% % \AND instead of \And before the third author name.

% % \vspace{-\rmSectionSpace}
% \author{%
%   David S.~Hippocampus\thanks{Use footnote for providing further information
%     about author (webpage, alternative address)---\emph{not} for acknowledging
%     funding agencies.} \\
%   Department of Computer Science\\
%   Cranberry-Lemon University\\
%   Pittsburgh, PA 15213 \\
%   \texttt{hippo@cs.cranberry-lemon.edu} \\
%   % examples of more authors
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \AND
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
% }
% % \vspace{-\rmSectionSpace}

% \begin{document}

% \maketitle

% %------------------------------------------- ABSTRACT ------------------------------------------------------%
% %-----------------------------------------------------------------------------------------------------------%
% \begin{abstract}

% Continual learning studies agents that learn from streams of tasks without forgetting previous ones while adapting to new ones. Two recent continual-learning scenarios have opened new avenues of research. In \emph{meta-continual learning}, the model is pre-trained to minimize catastrophic forgetting of previous tasks. In \emph{continual-meta learning}, the aim is to train agents for \emph{faster remembering} of previous tasks through adaptation. In their original formulations, both methods have limitations. We stand on their shoulders to propose a more general scenario where an agent must quickly solve new (out-of-distribution) tasks, while also requiring fast remembering. We show that current continual learning, meta-learning, meta-continual learning, and continual-meta learning techniques fail in this new scenario.
% We propose \textit{Continual-MAML}, an online extension of the popular MAML algorithm as a strong baseline for this scenario. We empirically show that \textit{Continual-MAML} is better suited to the new scenario than the aforementioned methodologies, as well as standard continual learning and meta-learning approaches.

% % Learning from non-stationary data remains a great challenge for machine learning. Continual learning addresses this problem in scenarios where the learning agent faces a stream of changing tasks. In these scenarios, the agent is expected to retain its highest performance on previous tasks without revisiting them while adapting well to the new tasks. Two new recent continual-learning scenarios have been proposed. In \emph{meta-continual learning}, the model is pre-trained to minimize catastrophic forgetting when trained on a sequence of tasks. In \emph{continual-meta learning}, the goal is \emph{faster remembering}, i.e., focusing on how quickly the agent recovers performance rather than measuring the agent's performance without any adaptation.
% % Both scenarios have the potential to propel the field forward. Yet in their original formulations, they each have limitations. As a remedy, we propose a more general scenario where an agent must quickly solve (new) out-of-distribution tasks, while also requiring fast remembering. We show that current continual learning, meta learning, meta-continual learning, and continual-meta learning techniques fail in this new scenario.
% % Accordingly, we propose a strong baseline: \textit{Continual-MAML}, an online extension of the popular MAML algorithm. In our empirical experiments, we show that our method is better suited to the new scenario than the methodologies mentioned above, as well as standard continual learning and meta learning approaches.


% \end{abstract}


% %------------------------------------------- INTRODUCTION -------------------------------------------------%
% %----------------------------------------------------------------------------------------------------------%
% \section{Introduction}
% \label{sec:intro}


% % A common assumption in machine learning is that the input to a learning algorithm consists of  independent and  identically distributed (i.i.d.) data. This assumption is violated in many practical applications handling non-stationary data distributions, including  robotics, autonomous driving cars, conversational agents  and other real-time applications, from sensor data analysis to stock market prediction, to name a few. Over the last few years, several methodologies were developed that relax the i.i.d.\ assumption. We focus on \emph{Continual learning} (CL), where the goal is to learn incrementally from a non-stationary data sequence involving different datasets or \emph{tasks}, while not forgetting previously acquired knowledge, a problem known as \emph{catastrophic forgetting}~\citep{mccloskey1989catastrophic}. 


% A common assumption in supervised machine learning is that data is independently and identically distributed (i.i.d.). This assumption is violated in many practical applications handling non-stationary data distributions, including robotics, autonomous driving, conversational agents, and other real-time applications. Over the last few years, several methodologies study learning from non i.i.d. data. We focus on \emph{continual learning} (CL), where the goal is to learn incrementally from a non-stationary data sequence involving different datasets or \emph{tasks}, while not forgetting previously acquired knowledge, a problem known as \emph{catastrophic forgetting}~\citep{mccloskey1989catastrophic}. 

% We draw inspiration from autonomous systems deployed in environments or domains that might differ from the ones they were (pre-)trained on. For instance, a robot pre-trained in a factory and deployed in homes where it will need to adapt to new domains and even solve new tasks. Likewise, a virtual assistant can be pre-trained on static datasets and deployed in a user's life to fit its personal needs. Further motivations can be found in time-series forecasting including market prediction, game playing, autonomous customer service, recommendation systems, and autonomous driving. These systems must adapt online to maximize their cumulative rewards~\citep{kaelbling1991foundations, kaelbling1993learning}. As a step in that direction, we propose a task-incremental scenario (OSAKA) where previous tasks reoccur and new tasks appear. We measure the cumulative accuracy of models instead of the (more) common final accuracy to evaluate how quickly models and algorithms adapt to new tasks and remember previous ones.


% % Continual learning is useful in various scenarios~\citep{Farquhar18}--unsupervised, supervised, and especially reinforcement learning, where the observed data can vary a lot between different locations in the environment~\citep{kaelbling1996reinforcement}. {\em Supervised continual learning} has become the most active area of recent CL research. Compared to reinforcement learning, it is much easier to study the forgetting problem in isolation when there is no credit assignment problem. As for unsupervised learning, finding good evaluations metric is still an open problem. Furthermore, supervised learning problems usually require less compute and memory resources, which enables researchers to iterate faster and lowers the bar entry. Accordingly, we keep the focus on supervised CL.


% \paragraph{Background} A common supervised CL scenario is \emph{task-incremental classification}, where classification datasets are presented to an online learner sequentially, one task at a time. For each task $T_t$ at iteration $t$, the data are sampled i.i.d.\ from their corresponding distribution $P_t({\bf x},y)$. In the task-incremental scenario models are evaluated by their average final performance across all tasks---after being trained on all tasks sequentially. 
% %The model must adapt to new tasks, learning to perform accurate classifications on them, while still retaining its predictive performance on previously learned tasks. 
% %In other words, CL methods are often evaluated using their (average) performance over all tasks after training on them in an incremental (sequential) fashion. 
% Several families of recent CL approaches use this setting, including regularization methods~\citep{kirkpatrick2017overcoming}, data replay~\citep{soltoggio2015short}, and dynamic architectures~\citep{rusu2016progressive}  (see \citet{lange2019continual} and \citet{Parisi18review} for comprehensive overviews).

% More recent approaches propose relaxing some constraints associated with task-incremental CL by combining CL and meta-learning. \emph{Continual-meta learning} (CML) focuses on \emph{fast remembering} or how quickly the model recovers its original performance on past tasks~\citep{He2019TaskAC}. \emph{Meta-continual learning} (MCL) uses meta-learning to learn not to forget~\citep{Javed2019Meta}. In this paper, we further extend the task-incremental setting and show empirical benefits compared to CML and MCL (see \cref{sec:experiments}).

% %Most recently, two approaches combine continual learning with meta learning to remove some of the constraints associated with task-incremental. 

% % \begin{comment}
% % Instead of focusing on avoiding forgetting, CML proposes to measure \emph{fast remembering} or how quickly the model recovers its original performance on past tasks. However, in its current formulation, CML still assumes that all previous knowledge must be stored in the model. This is achieved by applying CL methods on the meta parameters (the \emph{slow weights} in meta-learning terminology). In a study we show that this constraint hinders the model's ability to quickly adapt and learn new tasks whilst being computationally inefficient (see \cref{sec:experiments}).
% % \end{comment}

% % \begin{comment}
% % MCL, on the other hand, proposes a two-stage approach: 1) meta-learn a model with the explicit goal of not forgetting past knowledge (i.e., meta learn not to forget); followed by 2) a \emph{continual-learning stage} (referred to as ``CL time'') to evaluate the performance of the model on a stream of new examples from previous tasks (e.g.,\ training on a subset of MNIST classes and continually learning on a disjoint set of MNIST classes). Theses stages are analogous to the learning and active phase in robotics parlance~\citep{kaelbling1993learning}. MCL drastically reduces catastrophic forgetting when the data distribution is linearly separable in the pre-trained latent space, which is achieved in part by fixing the embedding space at CL time. In our study we show that fixed embeddings cannot handle out-of-distribution (OoD) tasks from similar datasets. (see \Cref{sec:experiments}). These results question the viability of current MCL in real-life applications.
% % \end{comment}
% %Therefore, we focus on models that can learn brand new tasks or behave plausibly in novel situations \citep{kaelbling1987architecture,kaelbling1992adaptable}.

% \paragraph{\newacron{}} We propose a more flexible and general scenario inspired by a pre-trained agent that must keep on learning new tasks after deployment.
% %---which is designed with challenging real-life applications in mind. We imagine an agent first pre-trained in a controlled environment and later deployed in the real world, where it faces new or unexpected situations. This scenario is relevant for many applications. For instance, in robotics, the agent is pre-trained in a factory and deployed in homes or in manufactures where it will need to adapt to new domains and maybe solve new tasks. Likewise, a virtual assistant can be pre-trained on static datasets and deployed in a user's life to fit its personal needs. Further motivations can be found in time series forecasting, e.g., market prediction, game playing, autonomous customer service, recommendation systems, autonomous driving, to name a few.
% In this scenario, we are interested in the cumulative performance of the agent throughout its lifetime~\cite{kaelbling1991foundations, kaelbling1993learning}.  (Standard CL reports the final performance of the agent on all tasks at the end of its \emph{life}.) To succeed in this scenario, agents need the ability to learn new tasks as well as quickly remember old ones.

% % \begin{comment}
% % \paragraph{\newacron{}} We expand the above CL frameworks towards a more flexible and general scenario---which is designed to be better suited for many challenging real-life applications. We imagine an agent, embedded or not, first pre-trained in a controlled environment and later deployed in the real world, where it faces new or unexpected situations. This scenario is relevant for many applications. For instance, in robotics, the agent is pre-trained in a factory and deployed in homes or in manufactures where it will need to adapt to new domains and maybe solve new tasks. Likewise, a virtual assistant can be pre-trained on static datasets and deployed in a user's life to fit its personal needs. Further motivations can be found in time series forecasting, e.g., market prediction, game playing, autonomous customer service, recommendation systems, autonomous driving, to name a few.
% % In this scenario, we are interested in the cumulative performance of the agent throughout its lifetime, as advocated in \citet{kaelbling1991foundations,kaelbling1993learning}. Differently, standard CL reports the agent's final performance on all tasks at the end of its \emph{life}. In order to succeed in this scenario, agents need the ability to learn new tasks as well as quickly remembering old ones. 
% % % something about how we dont care about the "asymptotic policy" the agent can reach upon convergence. 
% % \end{comment}
% We name our CL setting  \textit{\newsetting} (\newacron). The main characteristics of \newacron{} are that at deployment or CL time: 1) task shifts are sampled stochastically, 2) the task boundaries are unknown ({\em task-agnostic} setting), 3) the target distribution is context-dependent, 4) multiple levels of non-stationarity are used, and 5) tasks can be revisited. Furthermore, our evaluation of CL performance is different from the one commonly used in CL. We report the cumulative or online average performance instead of the final performance on all seen tasks. 

% Existing CL methods are not well-suited to \newacron. Methods such as EWC~\citep{kirkpatrick2017overcoming}, progressive networks~\citep{rusu2016progressive} or MCL~\citep{Javed2019Meta} require task boundaries. In contrast, task-agnostic methods (e.g. \citep{Aljundi17, zeno2018task, He2019TaskAC}) optimize for the final performance of the model and so resort to mechanisms that attempt to eliminate catastrophic forgetting. The extra computations resulting from the mechanisms hinder online performance and unnecessarily increase the computational footprint of the algorithms.

% To address the challenges of \newacron{}, we propose {\em Continual-MAML}, a baseline inspired by the meta-learning approach of MAML~\citep{finn2017model}. Continual-MAML is pre-trained via meta-learning. When deployed, Continual-MAML adapts the learned parameter initialization to solve new tasks. When a change in the distribution is detected, new knowledge is added into the learned initialization. As a result, Continual-MAML is more efficient and robust to distribution changes since it does not require computationally expensive optimizers like BGD~\citep{zeno2018task} or replay methods used in prior work~\citep{Chaudhry18,shin2017continual}.

% Using our \newacron~scenario, we compare the performance of Continual-MAML to recent and popular approaches from continual learning, meta-learning, and continual-meta learning. Across several datasets, we observe that Continual-MAML is better suited to \newacron{} than  prior methods from the aforementioned fields and thus provides an initial strong baseline. 

% To summarize, our contributions include: (1) \newacron{}, a new CL setting which is more flexible and general than previous ones. Related, we also propose a unifying scenario for discussing meta- and continual learning scenarios (\Cref{tbl:uni}); (2) the Continual-MAML algorithm, a new baseline that addresses the challenges of the \newacron{} setting; (3) extensive empirical evaluation of our proposed method%and the current literature in this new scenario
% ; and (4) a codebase for researchers to test their methods in the \newacron{} scenario.\footnote{\url{https://github.com/*****/*****}} 
% % \footnote{\url{https://github.com/ElementAI/osaka} \mytodo{anonymise}} 




% %---------------------------------------------- UNIFY ------------------------------------------------------%
% %-----------------------------------------------------------------------------------------------------------%
% \vspace{-\rmSectionSpace}
% \section{A unifying framework}
% \label{sec:setup}
% \vspace{-\rmSectionSpace}


% \newcommand{\cl}{\operatorname{CL}}
% \newcommand{\ctxt}{C}
% \newcommand{\loss}{\mathcal{L}}
% \newcommand{\world}{\mathcal{W}}
% \newcommand{\algo}{\mathcal{A}}
% \newcommand{\highlight}[1]{\textcolor{blue}{#1}}


% \begin{table*}[t]
%     % \begin{scriptsize}
%     \begin{tiny}
%     %\begin{sc}
%     \begin{center}
%     \resizebox{0.9\linewidth}{!}{%
%     \centerline{
%     \setlength{\tabcolsep}{6pt}
%     \renewcommand{\arraystretch}{1.7}
%     \begin{tabular}{ccccc}
%     \toprule
%         % \hline
%         & {\scriptsize Data} & {\scriptsize Fast} & {\scriptsize Slow} & {\scriptsize Eval}  \\
%         \midrule
%         { \scriptsize Supervised Learning} & $ S, Q \sim C $ & $ f_\theta = \algo(S) $ & --- & $ \loss(f_\theta, Q) $ \\
%         \midrule 
%         \makecell{\scriptsize Meta-learning} & \makecell{ $\{C_i\}_{i=1}^M \sim \world^M$ \\ $S_i, Q_i \sim C_i $ }& $ f_{\theta_i} = \algo_\phi(S_i)$ & $ \makecell{\nabla_\phi \loss( f_{\theta_i}, Q_i) \\ {\scriptstyle \forall i<N}} $ & $ \sum_{i=N}^M \loss(\algo_\phi(S_i), Q_i) $\\
%         %\midrule
%         \makecell{\scriptsize  Continual Learning} & $S_{1:T}, Q_{1:T} \sim C_{1:T}$ & $ f_\theta = \cl(S_{1:T}) $ & --- & $\sum_t \loss ( f_\theta, Q_t) $ \\
%         \midrule
%         \makecell{\scriptsize  Meta-Continual Learning} &  \makecell{ $ \{C_{i,1:T}\}_{i=1}^M \sim \world^M$ \\ $ S_{i, 1:T}, Q_{i, 1:T} \sim C_{i,1:T} $} & $f_{\theta_i} = \cl_\phi(S_{i,1:T}) $ &  \makecell{ $\nabla_\phi \sum_t \loss( f_{\theta_i} , Q_{i,t} )$ \\
%          ${\scriptstyle \forall i<N}$ } & $\sum_{i=N}^M\sum_t \loss (\algo_\phi(S_{i,1:T}), Q_{i,t}) $ \\
%         %\midrule 
%         \makecell{\scriptsize Continual-meta learning}  & $ S_{1:T}, Q_{1:T} \sim C_{1:T}$ & $f_{\theta_t} = \algo_\phi(\highlight{S_{t-1}})$& $\nabla_\phi \loss( f_{\theta_t}, S_t)$ & $ \sum_t \loss( \algo_\phi(S_t), Q_t )$\\ %$ \sum_t \loss( \algo_\phi(S_t), Q_t )$ \\
%         \midrule
%         \makecell{\scriptsize \newacron{}}  & $ Q_{1:T} \sim C_{1:T}$ & $f_{\theta_t} = \algo_\phi(\highlight{Q_{t-1}})$& $\nabla_\phi \loss( f_{\theta_t}, Q_t)$ &$ \sum_t \loss( f_{\theta_t}, Q_t )$ \\  
%         \bottomrule
%     \end{tabular}
%     %}
%     }}
%     \end{center}
%     %\end{sc}
%     % \end{scriptsize}
%     \end{tiny}
%     % \vspace{-\trimSize}
%     \vspace{-0.3cm}    
%     \caption{\textbf{A unifying framework} for different machine learning settings. Data sampling, fast weights computation and slow weights updates as well as evaluation protocol are presented with meta-learning terminology, i.e., the support set $S$ and query set $Q$. For readability, we omit OSAKA pre-training.}
%     \vspace{-0.4cm}   
%     \label{tbl:uni}
% \end{table*}
% % \vspace{-1cm}


% We introduce the concepts and accompanying notation that we will use to describe OSAKA in \Cref{sec:osaka}. These concepts provide a unifying framework---highlighted in \Cref{tbl:uni}---for expressing several important paradigms such as continual learning, meta-learning, and variants. 
% %We also discuss our proposed setting \newacron{} for continual learning, including the data generation process, our unifying framework, and the setting details.


% We begin by assuming a hidden context variable $C$ that determines the data distribution, e.g., the user's mood in a recommender system or an opponent's strategy in game playing. We use $\world$ to denote a finite set of all possible contexts. Given $C$, data can be sampled i.i.d.\ from $p(X|C)$. Different learning paradigms can be described by specializing the distribution $P(C)$. For example, in the classical setting data are sampled i.i.d.\ from $p(X|C)P(C)$ where $C$ could represent classes. 

% % In continual learning, the data distribution is non-stationary, and various CL scenarios arise from specific assumptions about this non-stationarity. Here we assume that data non-stationarity is caused by a hidden process $\{C_t\}_{t=1}^T$, where $C_t$ is the context at time $t$. $C$ in continual learning can be the task label, e.g., in Permuted MNIST, disjoint MNIST/CIFAR10~\cite{kirkpatrick2017overcoming}. It could also be the class label in the incremental classification setting~\cite{rebuffi2017icarl}. $\{C_t\}_{t=1}^T$ is usually assumed to be an ordered list of the tasks/classes. 

% %We propose a unifying notation to highlight the differences between several relevant machine-learning paradigms. In particular, we compare continual learning with meta-continual learning, continual-meta learning, meta-learning, and supervised learning (See \Cref{tbl:uni}).

% We use terminology from meta-learning and introduce a \textit{support set} $S$ and a \textit{query set} $Q$ to denote the meta-training and meta-test sets~\citep{vinyals2016matching}, respectively. These sets are usually composed of $n$ i.i.d.\ samples $X_i=(x_i,y_i)$, generated conditionally from the context $C_i$. In some paradigms, including supervised learning, the target distribution is fixed, i.e. $p(y|x)=p(y|x,c)$. We refer to the setting where the equality does not hold as having \textit{context-dependent targets}. We define a learning algorithm $\algo$ as a functional taking $S$ as input and returning a predictor $f_\theta$, with $\theta$ parameters describing the behavior of the predictor, i.e.\ $f_\theta = \algo(S)$. We also define a loss function $\loss(f_\theta, Q)$ to evaluate the predictor $f_\theta$ on the query set $Q$.

% In {\bf meta-learning}, $C$ represents the task descriptor or task label, and both meta-training and meta-testing sets are sampled i.i.d.\ from $P(X| C)$. E.g., applied to $N$-shot classification, the task descriptor would specify the $N$ classes which have to be discriminated. Targets are context-dependent in this learning paradigm.

% A meta-learning algorithm $\algo_\phi$ adapts its behavior by learning the parameters $\phi$. It samples $M$ i.i.d.\ pairs of $S$ and $Q$ from a distribution over contexts $\world^M$, that is, $\{C_i\}_{i=1}^M \sim \world^M$ and $(S_i, Q_i) \sim X_i\mid C_i$. Assuming that the learning process is differentiable, the parameters $\phi$ can be adjusted using the gradient from evaluation on the query set, $\nabla_\phi \loss( \algo_\phi(S_i), Q_i)$. For the final evaluation, $\phi$ is learned on the sets $(S_i, Q_i)$, where $i<N<M$ and the evaluation is done using $ \sum_{i=N}^M \loss(\algo_\phi(S_i), Q_i) $.

% In task-incremental {\bf continual learning}, the data distribution is non-stationary, and various CL scenarios arise from specific assumptions about this non-stationarity. Here we assume that data non-stationarity is caused by a hidden process $\{C_t\}_{t=1}^T$, where $C_t$ is the context at time $t$. $C$ in continual learning can be the task label, e.g., in Permuted MNIST, disjoint MNIST/CIFAR10~\cite{kirkpatrick2017overcoming}. It could also be the class label in the incremental classification setting~\cite{rebuffi2017icarl}. Both frameworks have a fixed target distribution. $\{C_t\}_{t=1}^T$ is usually assumed to be an ordered list of the tasks/classes. 

% Continual learning algorithms work with a sequence of support sets, $S_{1:T}$, and a sequence of query sets, $Q_{1:T}$, obtained from a sequence of contexts, $C_{1:T}$. A continual learning algorithm $\cl$ transforms $S_{1:T}$ into a predictor $f_\theta$, i.e.\ $f_\theta = \cl(S_{1:T})$. The main difference with a conventional algorithm $\algo$ is that the support set is observed sequentially and cannot be fully stored in memory. The evaluation is then performed independently on each $Q_t$ (obtained in the same context as $S_t$): $\sum_{t=1}^T \loss( f_\theta, Q_t)$.


% {\bf Meta-continual learning} combines meta-learning and continual learning. A collection of $M$ sequences of contexts is sampled i.i.d.\ from a distribution over sequences of contexts, $\world^M$, i.e., $ \{ C_{i,1:T}\}_{i=1}^M \sim \world^M$ and $S_{i,1:T}, Q_{i,1:T} \sim
% X_{i,1:T}\mid C_{i,1:T}$. Next, the continual learning algorithm, $\cl_\phi$, can be learned using the gradient $\nabla_\phi \sum_t \loss( \cl_\phi( S_{i,1:T} ) , Q_{i,t} )$, for $i < N < M$ and evaluated on the remaining sets $\sum_{i=N}^M \sum_t \loss( \cl_\phi( S_{i,1:T} ) , Q_{i,t} )$. As in continual learning, the target distribution is fixed.


% {\bf Continual-meta learning} considers a sequence of datasets $S_{1:T}, Q_{1:T} \sim C_{1:T}$. At training or continual-learning time, $S_{1:T}$ is both used as a support and query set: $S_t$ is used as the query set and $S_{t-1}$ as the support. Predictions at time $t$ are made using $f_{\theta_t} = \algo_\phi(Q_{t-1})$. Since local stationarity is assumed, the model always fails on its first prediction when the task switches. Next, using $l_t = \loss(f_{\theta_t}, S_t)$, the learning of $\phi$ is performed using gradient descent of $\nabla_\phi l_t$. The evaluation is performed at the end of the sequence where $\algo_\phi$ recomputes fast weights using the previous supports and is tested on the query set, i.e., $\sum_t \loss( \algo_\phi(S_t), Q_t)$. Similar to meta-learning, continual-meta learning allows for context-dependent targets.

% %% ALGORITHMS
% \SetKwIF{If}{ElseIf}{Else}{if}{}{else if}{else}{end if}%
% \SetKwFor{While}{while}{}{end while}%

% \centerline{
% \scalebox{0.85}{
%     \begin{minipage}{0.55\linewidth}
%         \setlength{\textfloatsep}{3mm}
%         \begin{algorithm2e}[H]
%         \SetAlgoLined
%         \DontPrintSemicolon
%         \textbf{Require:}  $P(\mathcal{C}_\text{pre})$, $P(\mathcal{C}_\text{cl})$: distributions of contexts\\
%         \textbf{Require:}  $\alpha$: non-stationarity level \\
%         \textbf{Initialize:} $\theta$: Model \\
%         \While{ pre-training }{
%         Sample a context $\mathcal{C} \sim P(\mathcal{C}_\text{pre})$ \\
%         Sample data from context $X, Y \sim P(X, Y |\mathcal{C})$ \\
%         Update $\theta_0$ with $X, Y$
%         }
%         \textbf{Initialize:} $\theta_0 \gets \theta$ \\   
%         \While{ continually learning }{
%             Sample current context $\mathcal{C}_t \sim P(\mathcal{C}_\text{cl} | \mathcal{C}_{t-1}, \alpha)$ \\
%             Sample data from context $X_t, Y_t \sim P(\mathcal{C}_t)$ \\
%             % Predict $\hat{Y_t} = f_{\theta_t}(X_t)$ \\
%             Incur loss $\mathcal{L}\big(\theta_{t-1}(X_t), Y_t\big)$ \\
%             % Obtain targets $Y$; Update $\theta_t$ with $X_t,Y_t$ at discretion \\
%             Update $\theta_t$ with $X_t,Y_t$ at discretion \\
%             $t \gets t+1$ \\
%         } 
%             \caption{OSAKA}
%         \label{algo:osaka}
%         \end{algorithm2e}
%     \end{minipage}
%     \hspace{2em}
%     \begin{minipage}{0.55\linewidth}
%         \setlength{\textfloatsep}{3mm}
%         \begin{algorithm2e}[H]
%             \SetAlgoLined
%             \DontPrintSemicolon
%             \textbf{Require:} $\eta, \gamma, \lambda$: learning rate, hyperparameters \\
%             ...\\
%             \setcounter{AlgoLine}{14}
%             \While{ continually learning }{
%                 $\mathcal{C}_t \sim P(\mathcal{C}_\text{cl} | \mathcal{T}_{t-1})$ \\
%                 $X_t, Y_t \sim P(\mathcal{C}_t)$ \\
%                 $\mathcal{L}\big(f_{\theta_{t-1}}(X_t), Y_t\big)$ \\
%                 $\tilde{\theta_t} \gets \phi - \phi_\eta \nabla_\phi \mathcal{L}\big(f_\phi(X_t), Y_t\big)$ \\
%                 \uIf{$\mathcal{L}\big(f_{\theta_{t-1}}(X_t), Y_t\big) - \mathcal{L}\big(f_{\tilde{\theta_{t}}}(X_t), Y_t\big) < \gamma$}{
%                 %  \# No context shift detected \\
%                 $\theta_t \gets \theta_{t-1} - \phi_\eta \nabla_\theta \mathcal{L}\big(f_{\theta_{t-1}}(X_t), Y_t\big)$ \\
%                 }
%               \uElse{
%                 %  \# Task boundary detected \\
%                 % $\eta_t \gets  \eta \lambda  \mathcal{L}\big(f_{\theta_{i-1}}(X_i), Y_i\big)$ \\
%                 $\eta_t \gets  \eta  g_\lambda \big( \mathcal{L}\big(f_{\theta_{i-1}}(X_i), Y_i\big) \big)$ \\
%                 $\phi \gets \phi - \eta_t \nabla_\phi \mathcal{L}\big(f_{\theta_{t-1}}(X_t), Y_t\big)$ \\
%                 $\theta_t \gets \phi - \phi_\eta \nabla_\phi \mathcal{L}\big(f_\phi(X_t), Y_t\big)$  \\
%                 }
%                 $t \gets t+1$ \\
%             }
%             \caption{Continual-MAML at CL time}
%         \label{algo:cmaml}
%         \end{algorithm2e}
%     \end{minipage}
% }
% }

% %---------------------------------------------- OSAKA ------------------------------------------------------%
% %-----------------------------------------------------------------------------------------------------------%
% % \vspace{-\rmSectionSpace}
% \section{Online FaSt Adaptation and Knowledge Accumulation (OSAKA)} 
% \label{sec:osaka}
% % \vspace{-\rmSectionSpace}

% % \vspace{-2cm}



% We propose \newacron{}, a new approach to continual learning that lifts some of constraints of current task-incremental approaches~\cite{kirkpatrick2017overcoming, Javed2019Meta, Aljundi2019Online}. \newacron{} is aligned with the use case of deploying a pre-trained agent in the real world, where it must adapt quickly to new situations and even learn new concepts when needed. In particular, \newacron{} proposes a scenario for evaluating such agents. 

% To materialize such an evaluation \newacron{} combines different ideas: 1) agents start in a pre-training stage before continual-learning time; 2) it provides a mechanism for proposing both old and new tasks to agents where the boundaries between tasks remain unobserved to them; 3) it evaluates agents using their cumulative performance (e.g. accuracy) to measure their capacity to adapt to new tasks. 
% This evaluation implicity allows for agents to forget which may enable faster and more efficient adaptation. For instance, partially forgetting an infrequent task allows the agent to re-allocate modeling capacity to tasks that are encountered more frequently. We detail each idea below including how they depart from current work and also provide a procedural view of \newacron{} in \Cref{algo:osaka}. 



% %To enable the evaluation adaptation to new tasks, \newacron{} 
% %Current methods force models to retain their performance on all previously seen tasks. This is an an unrealistic constraint, particularly with limited computational resources~\cite{kaelbling1991foundations, kaelbling1993learning}. 
% %This is An application deployed in the real world may be evaluated by its real-time decision making performance~\cite{kaelbling1991foundations, Alet2018ModularM}. Further, previous settings focus on optimizing the final performance on all tasks.   


% {\bf Task revisiting.} 
% Standard CL methods incrementally learn strictly new tasks. However, most CL applications require revisiting previous tasks. Accordingly, \newacron{} assumes task revisiting as \emph{recurrent concept drift}~\cite{gama2014survey} where the process $\{C_t\}_{t=1}^T$ follows a Markov chain with transition probabilities $P(C_t|C_{t-1})$ (\cref{algo:osaka}, L11). Further, these transitions allow $C_t$ to switch back and forth from old tasks to OoD tasks. In this setting, models have to if the new task is OoD or known.
% %This assumption brings us closer to real applications such as reinforcement learning where the states follow a Markov chain given the previous state and action~\cite{kaelbling1996reinforcement}.
% % Compared to previous settings, this not only introduces a dependency between consecutive context variables but also allows the agent to revisit previous tasks. 


% {\bf Task agnostic.} 
% In \newacron{}, the task boundaries or context shifts are unobserved, and the agent must infer the current task or context $C_t$. This is called task-agnostic (or task-free) CL~\cite{Aljundi2019TaskFreeCL,Aljundi2019Gradient, zeno2018task, He2019TaskAC, lesort2019continual}. It provides a more realistic scenario since in many real-worlds signals indicating task shifts do not exist.% real-world agents. %since in the real-world agents may not know about task shifts.
% %Most CL works assume $C$ to be available for training~\cite{kirkpatrick2017overcoming, Nguyen17, lopez2017gradient}, which is unrealistic in many real applications, e.g., an embedded agent in a changing environment. Thus, . 

% {\bf Controllable non-stationarity.}
% \newacron{} provides control, through a hyperparameter, over the level of non-stationarity of the Markov chain. A stream is $\alpha$-locally-stationary when $P(C_t\!=\!c | C_{t-1}\!=\!c)\!=\!\alpha$. Namely, the data distribution is stationary within a local time window. Control over $\alpha$ enables exploring environments with different levels of non-stationarity to test algorithmic robustness.
% %The non-stationarity level of standard CL is often provided through the dataset sizes and the number of classes per task. Past works then design algorithms tailored to these levels of non-stationarity. Furthermore, real-life applications often operate on locally stationary data distributions, e.g., an autonomous vehicle navigating specific weather, a recommendation system dealing with users with time-varying interest \cite{hidasi2015session}, or an embedded agent doing a specific task for a while \citep{lomonaco2019continual,Padakandla2019ReinforcementLI}. The non-stationarity of the data, however, differ between tasks.


% {\bf Context-dependent targets.} 
% In standard CL, $p(x)$ shifts over time, but not the target distribution $p(y|x)$. Extending \cite{He2019TaskAC}, OSAKA allows for context-dependent targets (\cref{algo:osaka}, L12) making it more flexible and more aligned with our use-cases (\Cref{sec:intro}) or partially-observable environments. The characteristics mentioned so far are inspired by Hidden-Mode Markov Decision Processes~\citep{choi2000hidden}.
% % It is important to mention that some learning paradigms are more flexible w.r.t the target distribution. In supervised learning, $p(y|x)=p(y|x,c)$. In CL, this is true as well. Only $p(x)$ changes through time but the mapping $p(y|x)$ is fixed. The same can be said about MCL. In meta-learning and CML, however, $p(y|x,c) \neq p(y|c)$. This flexibility is needed, e.g., in partially observable environments, or any setting where predictions are dependent on a context. For the rest of this paper, we refer to this specificity as COOL\_NAME.



% \paragraph{Pre-training.}
% In many current settings~\cite{kirkpatrick2017overcoming, He2019TaskAC}, the agent begins learning from randomly-initialized parameters. However, it is unrealistic to deploy an agent without any world knowledge~\cite{lesort2019continual,lomonaco2019fine}, in part, since real-life non-i.i.d.\ training is difficult to learn. Further, in many domains, ample pre-training data can be leveraged. \newacron{} proposes a two-stage approach where agents start in a \emph{pre-training phase} (\cref{algo:osaka}, L4-L8) and then move to a \textit{deployment phase} (\cref{algo:osaka}, L10-L16) also known as continual-learning time. 



% \paragraph{Out-of-distribution tasks.} 
% Current settings that permit pre-training then continually learn tasks sampled from the same data distribution~\cite{Javed2019Meta, beaulieu2020learning}. In contrast, in \newacron{} the model has to learn online tasks sampled from new distributions not encountered at pre-training (see \cref{ssec:datasets} for details)). This setting is more realistic since an agent will encounter unexpected situations in real life requiring the algorithm to update its representations. 
% % by learning new discriminative features or new policies. 
% %For instance, this behavior could arise when an embedded agent learns to manipulate a new object or tool, or a virtual teacher learns a new concept.



% \paragraph{Online Evaluation} 
% Current settings call for methods to retain their performance on all previously seen tasks. This is an unrealistic constraint, particularly under limited computational resources~\cite{kaelbling1991foundations, kaelbling1993learning}. Instead of measuring the final performance of the model, \newacron{} measures the online cumulative performance which better suits non-stationary environments. Models are evaluated with $\sum_{t=1}^T{\mathcal{L}(f_{\theta_t},Q_t)}$ where $\mathcal{L}$ can be any metric (\cref{algo:osaka}, L13). This is similar to evaluating the (undiscounted) sum of rewards in reinforcement learning and also to evaluating regret~\citep{berry1985bandit} in online learning albeit without the burden of computing the performance of an optimal model. %Current methods force models to retain their performance on all previously seen tasks. This is an unrealistic constraint, particularly with limited computational resources~\cite{kaelbling1991foundations, kaelbling1993learning}. 
% %, which would be impossible in our case.


% %---------------------------------------------- METHODOLOGY ------------------------------------------------%
% %-----------------------------------------------------------------------------------------------------------%
% \vspace{-0.05cm}
% \section{Continual-MAML}
% \label{sec:method}
% \vspace{-0.05cm}


% % \vspace{-0.4cm}
% \begin{figure*}[b]
%     \centering
%     \includegraphics[trim={2cm 1cm 1cm 1cm},clip,width=0.90\linewidth]{figures/model.png}
%     \label{fig:problem_formulation}
%     \vspace{-0.12cm}
%     \caption{ \textbf{Continual-MAML} first pre-trains with MAML, obtanining $\phi$. At continual-learning time, the model adapts $\phi$ to new distributions. The algorithm retrains its slow weights $\phi$ when it detects an OoD task to add new knowledge to the model. 
%     % The figure is inspired from the one found in \citet{finn2017model}.}
%     This figure is inspired from the one found in \cite{finn2017model}.}
%     \vspace{-0.12cm}
%     \label{fig:cartoon}
% \end{figure*}

% We propose Continual-MAML (see \cref{fig:cartoon}), a CL baseline based on MAML~\cite{finn2017model} that can cope with the challenges of \newacron{}. Continual-MAML (see \cref{algo:cmaml} or its complete version \cref{algo:cmaml_full} in \cref{app:algo}) consists of two stages: pre-training and continual learning. 


% The pre-training phase consists of MAML. That is, meta-learning model parameters such that a small number of gradient steps on a small new task will produce good generalization performance on that task (\cref{algo:cmaml_full}, L6--13). Specifically, the model adapts its initial weights $\phi$ to multiple tasks in the inner loop, obtaining $\theta$. Then it updates the initialization $\phi$ in the outer loop. Note that the inner loop learning rate is meta-learned ($\phi_\eta$ in \cref{algo:cmaml_full}, L10).

% At CL time (\cref{algo:cmaml}), the inner loop optimization adapts the model to the current task. Specifically, the model uses current data $X_t,Y_t$ to obtain fast weights $\theta_t$ (\cref{algo:cmaml}, L21). Assuming that the data is locally stationary, it makes a prediction on the following data $X_{t+1}$ and incurs a loss (\cref{algo:cmaml}, L18). In the case of a sudden distribution shift, the model will fail at its first prediction because its fast weights $\theta_t$ are not suited for the new task yet, but it will have recovered by the next. The recovery is achieved by learning new fast weights $\theta_{t+1}$ once the algorithm gets feedback on its prediction (\cref{algo:cmaml}, L25). Note that for some real-life applications, this feedback could be delayed~\cite{kaelbling1996reinforcement}. Finally, to accumulate new knowledge, we further update the meta parameters $\phi$ on the incoming data as well (\cref{algo:cmaml}, L24).

% We also propose two features to improve Continual-MAML's performance. First, the algorithm must update its knowledge only when it is solving an OoD task. Accordingly, we introduce a hyperparameter $\lambda$ that controls the behavior of the algorithm between never training on the incoming data at CL time to always training (MAML and C-MAML in \Cref{sec:experiments}). Specifically, when $\mathcal{L}(f_{\theta_{t-1}}(X_t), Y_t)\!>\!\lambda$, new knowledge is incorporated through outer loop optimization of the learned initialization. This mechanism is exemplified in \cref{fig:cartoon}. To obtain a smoother interpolation between behaviors, we opted for a soft relaxation of the mechanism (\cref{algo:cmaml}, L23) where $g_\lambda: \mathbb{R} \rightarrow (0,1)$.  We call this first feature \textit{\firstFeature{}} (\firstFeatureAcron{}). 

% Second, to further leverage the local stationarity of OSAKA, we introduced a mechanism that keeps fine-tuning the fast weights $\theta$ (\cref{algo:cmaml}, L21) until a context shift or task boundary is detected. The simple yet effective context shift detection mechanism works by monitoring the difference in loss with respect to the previous task and is controlled by a hyperparameter $\gamma$ (\cref{algo:cmaml}, L20). We call this second feature \textit{\secondFeature{}} (\secondFeatureAcron{}). An ablation of both mechanisms and an hyperparameter sensitivity analysis are provided in \cref{ssec:results} and \cref{app:hparam_analysis}, respectively.

% As a result, different from previous CL literature, the proposed algorithm benefits from fast adaptation, dynamic representations, task boundary detection, and computational efficiency, as we describe next.


% \paragraph{Fast Adaption} During pre-training, Continual-MAML learns a weight initialization that adapts fast to new tasks. This is different from CL methods that focus on incorporating as much knowledge as possible into one representation that has to maximize performance in a multi-task regime. 


% \paragraph{Dynamic representations} In \newacron{}, significant distribution shifts occur periodically. As shown in \cref{sec:experiments}, models that require a fixed representation would fail to adapt. Instead, Continual-MAML, equipped with \firstFeatureAcron{}, detects OoD data and then learns new knowledge using outer-loop optimization. 


% \paragraph{Computational efficiency} As described by \citet{Farquhar18}, CL agents should operate under restricted computational resources since remembering becomes trivial in the infinite-resource setting. Continual-MAML satisfies this desideratum by allowing the agent to forget (to some extent) and re-allocate parametric capacity to new tasks. Likewise, no computationally expensive mechanisms, such as replay \cite{Chaudhry19}, or BGD \cite{zeno2018task,He2019TaskAC}, are used to alleviate catastrophic forgetting in our method.

% \paragraph{Task boundary detection} Continual-MAML detects context shifts which not only help to condition its predictive function on more datapoints (\secondFeatureAcron{}), it also avoids mixing gradient information from two different distributions.







% % }
   
% %   \scalebox{0.9}{
% %     \begin{minipage}{0.6\textwidth}
% %     \centering
% %     \begin{scriptsize}
% %     \begin{sc}
% %         \setlength{\tabcolsep}{1.6pt}
% %         \centering
% %         \begin{tabular}{lcccccc}
% %         \toprule
% %             & \multicolumn{2}{c}{pre-train} & \multicolumn{4}{c}{retrain} \\
% %           \cmidrule(l{2pt}r{2pt}){2-3}
% %           \cmidrule(l{2pt}r{2pt}){4-7}
% %             model & MAML & ANIL &  MAML  & SGD  & BGD & KWTO/AP \\
% %             \midrule
% %             Online ADAM                      & $\times$ & $\times$ & $\times$ & $\surd$  & $\times$ & $\times$ \\
% %             Fine Tuning                     & $\times$ & $\surd$  & $\times$ & $\surd$  & $\times$ & $\times$ \\
% %             BGD \citep{zeno2018task}        & $\times$ & $\times$ & $\times$ & $\times$ & $\surd$  & $\times$ \\
% %             MAML \citep{finn2017model}      & $\surd$  & $\times$ & $\times$ & $\times$ & $\times$ & n/a  \\
% %             ANIL \citep{raghu2019rapid}     & $\times$ & $\surd$  & $\times$ & $\times$ & $\times$ & n/a  \\ 
% %             MetaBGD \citep{He2019TaskAC}    & $\times$ & $\times$ & $\surd$  & $\times$ & $\surd$  & $\times$ \\
% %             MetaCOG \citep{He2019TaskAC}    & $\times$ & $\times$ & $\surd$  & $\times$ & $\surd$  & $\times$ \\
% %             Continual-MAML                  & $\surd$  & $\times$ & $\surd$  & $\times$ & $\times$ & $\surd$  \\
% %             \bottomrule
% %         \end{tabular}
% %     \end{sc}
% %     \end{scriptsize}
% %     % \vskip -0.1in
% %     \captionof{table}{\textbf{Baseline comparison.} Columns 2--3 contain pre-training algorithms. Columns 4--7 show training algorithms at continual learning time. KWTO and AP stand for \textit{knowing what to train on} and \textit{adaptation phase}, respectively.}
% %     \label{tab:baselines}
% %     \end{minipage}
% % } 

% %------------------------------------------- RELATED ------------------------------------------------------%
% %----------------------------------------------------------------------------------------------------------%
% \vspace{-\rmSectionSpace}
% \section{Related Work}
% \label{sec:related_work}
% \vspace{-\rmSectionSpace}

% Continual Learning (CL) \citep{mccloskey1989catastrophic,thrun1995lifelong} has evolved towards increasingly challenging and more realistic evaluation protocols. The first evaluation frameworks \citep{Goodfellow13,kirkpatrick2017overcoming} were made more general in \cite{zeno2018task,Aljundi2019TaskFreeCL} via the removal of the known task boundaries assumption. Later, \cite{He2019TaskAC} proposed to move the focus towards \textit{faster remembering}, or continual-meta learning (CML), which measures how quickly models recover performance rather than measuring the models' performance without any adaptation. \newacron{} builds upon this framework to get closer to real-life applications of CL, as explained in \cref{sec:osaka}. 

% \citet{Harrison2019ContinuousMW} propose a new CML framework and accompanying model (MOCA). OSAKA shares commonalities with this framework, but they are fundamentally different: it does not (1) allow context-dependent targets, (2) expose the algorithms to OoD tasks at CL time, (3) allow new unknown labels, nor (4) propose an update CL evaluation protocol.
% Further details are in \cref{app:moca}.


% % --------------------------------------------- EXPERIMENTS -----------------------------------------------------%
% %----------------------------------------------------------------------------------------------------------------%
% \vspace{-\rmSectionSpace}
% \section{Experiments}
% \label{sec:experiments}
% \vspace{-\rmSectionSpace}

% We study the performance of different baselines in the proposed \newacron{} setup. We first introduce the datasets, methods, and baselines, and then report and discuss experimental results and observations. 

% \vspace{-\rmSubsectionSpace}
% \subsection{Experimental setup}
% \label{ssec:datasets}
% \vspace{-\rmSubsectionSpace}

% %%% Figure: Datasets

% % \begin{wrapfigure}[20]{l}[1cm]{0.5\textwidth}
% %     \centering
% %     \includegraphics[trim={3cm 3cm 3cm 3cm},clip,width=0.5\textwidth]{figures/omniglot2.png}
% %     % \vspace{-0.5cm}
% %     \includegraphics[width=0.5\textwidth]{figures/synbols3.png}
% %     % \vspace{-0.5cm}
% %     \includegraphics[trim={0.25cm 0.25cm 0.25cm 0.5cm},clip,width=0.5\textwidth]{figures/tiered.png}
% %     % \vspace{-0.7cm}
% %     \label{fig:datasets}
% %     \caption{\textbf{Benchmarks.} We evaluate our setup on three different benchmarks, each one depicted in one row: Omniglot/MNIST/FashionMNIST, Synbols, and Tiered-ImageNet.} 
% % \end{wrapfigure}




% For all datasets we study two different levels of non-stationarity at CL time, $\alpha$ values of 0.98 and 0.90. Unless otherwise stated the continual-learning episodes have a length of 10,000 timesteps; the probability to visit the pre-training distribution and to visit one of the OoD ones is 0.5 and 0.25, respectively; we report the performance averaged over 20 runs per model, as well as the standard deviation. Statistical significance is assessed using a 95\% CI and highlighted in bold. Further experimental details are provided in \cref{app:exp_details}.
% %@Laurent, this is what I did https://www.socscistatistics.com/tests/studentttest/default.aspx

% \paragraph{Omniglot / MNIST / FashionMNIST}
% In this study, we pre-train models on the first 1,000 classes of Omniglot~\cite{lake2015human}. At CL time, the models are exposed to the full Onniglot dataset, and two out-of-distribution datasets: MNIST~\cite{lecun-mnisthandwrittendigit-2010} and FashionMNIST~\cite{xiao2017fashion}. Concerning the reported performance, MNIST is a simpler dataset than Omniglot, and FashionMNIST is the hardest. During CL time, the tasks switch with probability $1 \!- \!\alpha$. For this study, we sample 10-way 1-shot classification tasks.

% \paragraph{Synbols} In this study, models are pre-trained to classify characters from different alphabets on randomized backgrounds~\cite{lacoste2018uncertainty}. Tasks consist of 4 different symbols with 4 examples per symbol. During CL time, the model is exposed to a new alphabet. Further, the model will have to solve the OoD task of font classification, where the input distribution does not change, only its mapping to the output space. The font classification task consists of 4 different fonts with 4 symbols per font.

% \paragraph{Tiered-ImageNet} Like Omniglot, Tiered-ImageNet~\cite{ren2018meta}  groups classes into super-categories corresponding to higher-level nodes in the ImageNet \cite{deng2009imagenet} hierarchy (we use 20/6/8 disjoint sets for training/validation/testing nodes). We use these higher-level splits to simulate a shift of distribution. We follow the original splits, where the test set contains data that is out of the training and validation distributions. Thus, we use their training set for pre-training, and introduce their validation and test sets at CL time. We refer to them as train, test and OoD in \cref{tab:tiered}, respectively. Since only one of the two introduced sets is OoD, we increase its probability of being sampled to 0.5, in accordance to the previous benchmarks. This experiment uses 20,000 steps (twice as the others).
% % Thus, at pre-training time, the model is presented with 14 high-level categories from the original training split. At CL time, we use six new super-categories from the original validation split, as well as the remaining six categories from training. Since there is only one new set of categories at CL time, the probability of visiting it is 0.5. 


% \vspace{-\rmSubsectionSpace}
% \subsection{Baselines}
% \label{ssec:baselines}
% \vspace{-\rmSubsectionSpace}

% \cref{app:baselines} compares the main features of the baselines we benchmark in the \newacron{} setting. For meta-learning methods, ADAM \cite{kingma2014adam} and SGD are used for the outer and inner updates, respectively. 

% \paragraph{Online ADAM and Fine Tuning.} We use ADAM without and with pre-training as a lower bounds.

% % \paragraph{Online ADAM. } We use ADAM without pre-training as a lower bound.

% % \paragraph{Fine Tuning.} To study the effect of pre-training, we pre-train the model and fine tune it at CL time.

% \paragraph{BGD \citep{zeno2018task}.} Bayesian Gradient Descent (BGD) is a continual learning algorithm that models the distribution of the parameter vector $\phi$ with a factorized Gaussian. Similarly to \cite{He2019TaskAC} we apply BGD during the continual learning phase. More details about this baseline are provided in \cref{app:bgd}.

% \paragraph{MAML~\citep{finn2017model}.} MAML consists of a pre-training stage and a fine-tuning stage. During pre-training, the model learns a general representation that is common between the tasks. In the fine-tuning stage, the model fine-tunes its layers to adapt to a new task.

% \paragraph{ANIL~\cite{raghu2019rapid}.} ANIL differs from MAML only in the fine-tuning stage. Instead of adapting all the network layers, ANIL adapts only the network's head towards the new task. The goal of this baseline is to show the problem with static representations in the continual learning setup. Therefore, ANIL is representative of meta-continual learning.

% \paragraph{MetaBGD and MetaCOG~\cite{He2019TaskAC}.} MetaBGD performs CML using MAML and BGD to alleviate catastrophic forgetting. MetaCOG introduces a per-parameter mask learned in the inner loop.



% \vspace{-\rmSubsectionSpace}
% \subsection{Experimental results}
% \label{ssec:results}
% \vspace{-\rmSubsectionSpace}



% \begin{figure} [t]
%   \begin{subfigure}[b]{0.33\textwidth}
%     % \includegraphics[trim={0.5cm 0.5cm 0.5cm 0.5cm}, width=\textwidth]{figures/online_acc_Omniglot_full_hd.png}
%     \includegraphics[trim={0.cm 0.cm 0.cm 0.cm}, width=\textwidth]{figures/online_acc_Omniglot_full_hd.png}
%   \end{subfigure}
%   %
%   \begin{subfigure}[b]{0.33\textwidth}
%     % \includegraphics[trim={0.5cm 0.5cm 0.5cm 0.5cm}, width=\textwidth]{figures/online_acc_MNIST_full_hd.png}
%     \includegraphics[trim={0.cm 0.cm 0.cm 0.cm}, width=\textwidth]{figures/online_acc_MNIST_full_hd.png}
%   \end{subfigure}
%   %
%   \begin{subfigure}[b]{0.33\textwidth}
%     % \includegraphics[trim={0.5cm 0.5cm 0.5cm 0.5cm}, width=\textwidth]{figures/online_acc_Fashion_full_hd.png}
%     \includegraphics[trim={0.cm 0.cm 0.cm 0.cm}, width=\textwidth]{figures/online_acc_Fashion_full_hd.png}
%   \end{subfigure}
%   \caption{\textbf{Omniglot / MNIST / FashionMNIST experiment} in the $\alpha \! = \! 0.90$ regime. Standard error is computed with 20 runs. Online ADAM and Fine Tuning lie below of the graph.}
%   \label{fig:omniglot}
% \end{figure}


% %%%% RESULTS on synbols
% \setlength{\tabcolsep}{0.85pt}
% %\renewcommand{\arraystretch}{1}
% \begin{table*}[ht]
%   %\vskip 0.15in
%   %\begin{tiny}
%   \centering
%   \centerline{
%   \begin{scriptsize}
%   \begin{sc}
%   %\resizebox{\textwidth}{!}{%
%     \begin{tabular}{l|cccc|cccc}
%     \toprule
%     & \multicolumn{4}{c|}{$\alpha=0.98$} & \multicolumn{4}{c}{$\alpha=0.90$} \\
%     model & Total & Prev. Alph. & New Alph. & Font Class. & Total & Prev. Alph. & New Alph. & Font Class. \\ 
%     \midrule 
%     %\hline
%         Online ADAM & 59.6  \std{1.5} & 63.7  \std{2.3} & 59.5  \std{3.7} & 50.7  \std{2.9} & 27.5  \std{0.8} & 28.3  \std{1.1} & 26.3  \std{0.9} & 26.9  \std{0.7} \\
%         Fine Tuning & 64.0  \std{2.0} & 69.6  \std{2.1} & 63.0  \std{3.6} & 52.9  \std{2.8} & 26.6  \std{1.8} & 27.0  \std{2.4} & 26.2  \std{1.5} & 26.1  \std{1.2} \\
%         MAML \citep{finn2017model} & 71.2  \std{2.8} & 90.3  \std{0.8} & 65.7  \std{1.5} & 37.9  \std{1.1} & 69.3  \std{0.9} & 86.3  \std{0.5} & 64.3  \std{0.7} & 40.4  \std{0.7} \\
%         ANIL \citep{raghu2019rapid} & 69.4  \std{1.9} & 91.3  \std{0.8} & 59.0  \std{1.6} & 33.2  \std{1.0} & 70.2  \std{0.8} & \bf88.4  \std{0.4} & 68.7  \std{0.6} & 35.1  \std{0.5} \\
%         BGD \citep{zeno2018task} & 68.3  \std{1.4} & 73.6  \std{2.3} & 69.7  \std{3.0} & 56.1  \std{3.5} & 33.9  \std{1.3} & 36.7  \std{1.6} & 32.0  \std{1.9} & 30.3  \std{0.9} \\
%         % MAML & 71.2  \std{2.8} & 90.3  \std{0.8} & 65.7  \std{1.5} & 37.9  \std{1.1} & 69.3  \std{0.9} & 86.3  \std{0.5} & 64.3  \std{0.7} & 40.4  \std{0.7} \\
%         MetaCOG \citep{He2019TaskAC} & 68.3  \std{1.7} & 73.6  \std{1.7} & 69.6  \std{2.8} & 56.8  \std{2.8} & 34.6  \std{1.3} & 37.1  \std{1.8} & 33.5  \std{2.4} & 30.5  \std{1.0} \\
%         MetaBGD \citep{He2019TaskAC} & 72.5  \std{1.6} & 77.8  \std{1.8} & 73.6  \std{1.7} & 58.8  \std{3.5} & 60.3  \std{0.4} & 65.8  \std{0.7} & 62.2  \std{1.4} & 47.8  \std{1.4} \\
%         % MetaCOG & 68.3  \std{1.7} & 73.6  \std{1.7} & 69.6  \std{2.8} & 56.8  \std{2.8} & 34.6  \std{1.3} & 37.1  \std{1.8} & 33.5  \std{2.4} & 30.5  \std{1.0} \\
%         % fine\_tuning & 64.0  \std{2.0} & 69.6  \std{2.1} & 63.0  \std{3.6} & 52.9  \std{2.8} & 26.6  \std{1.8} & 27.0  \std{2.4} & 26.2  \std{1.5} & 26.1  \std{1.2} \\
%         % online\_sgd & 59.6  \std{1.5} & 63.7  \std{2.3} & 59.5  \std{3.7} & 50.7  \std{2.9} & 27.5  \std{0.8} & 28.3  \std{1.1} & 26.3  \std{0.9} & 26.9  \std{0.7} \\
%         \midrule %\hline
%         C-MAML & 74.4  \std{1.4} & 79.4  \std{1.1} & 76.3  \std{2.6} & 61.6  \std{3.1} & 61.2  \std{2.5} & 66.5  \std{3.1} & 62.9  \std{2.8} & 49.3  \std{1.7} \\
%         C-MAML + pre. & 78.4  \std{1.0} & 86.6  \std{1.0} & 78.2  \std{1.4} & 60.9  \std{2.6} & 73.3  \std{1.2} & 82.0  \std{1.1} & 75.0  \std{1.6} & 53.8  \std{1.5} \\
%         C-MAML + pre. + \firstFeatureAcron{} & 74.8  \std{4.0} & 81.6  \std{6.2} & 75.5  \std{4.5} & 59.5  \std{3.2} & 72.8  \std{0.9} & 81.4  \std{1.2} & 74.4  \std{1.3} & 54.4  \std{1.6} \\
%         C-MAML + pre. + \firstFeatureAcron{}+ \secondFeatureAcron{} & \bf 86.3  \std{0.8} & \bf 93.4  \std{0.6} & \bf 86.7  \std{1.8} & \bf 72.0  \std{2.4} & \bf 76.3  \std{0.8} & 84.9  \std{0.7} & \bf 76.4  \std{1.5} & \bf 58.5  \std{1.4} \\
%         \bottomrule
%     \end{tabular}
%   %}
%   \end{sc}
%   \end{scriptsize}
%   }
%   %\end{tiny}
%   \vspace{-0.12cm}
%   \caption{\textbf{Synbols experiment}}
%   \vspace{-0.15cm}
% \label{tab:synbols}
% \end{table*}



% %%%% RESULTS on Tiered
% \setlength{\tabcolsep}{2.6pt}
% %\renewcommand{\arraystretch}{1}
% \begin{table*}[ht]
%   %\vskip 0.15in
%   %\begin{tiny}
%   \centering
%   \centerline{
%   \begin{scriptsize}
%   \begin{sc}
%   %\resizebox{\textwidth}{!}{% 
%     \begin{tabular}{l|cccc|cccc}
%     \toprule
%     & \multicolumn{4}{c|}{$\alpha=0.98$} & \multicolumn{4}{c}{$\alpha=0.90$} \\
%     model & Total & Train & Test & OoD & Total & Train & Test & OoD \\ 
%     \midrule
%     %\hline
%         Online ADAM & 44.5  \std{1.7} & 43.9  \std{2.1} & 44.6  \std{2.2} & 44.6  \std{2.1} & 22.7  \std{0.2} & 22.7  \std{0.4} & 22.6  \std{0.4} & 22.7  \std{0.3} \\
%         Fine Tuning & 44.6  \std{1.5} & 43.8  \std{2.8} & 44.1  \std{2.1} & 45.2  \std{1.8} & 22.6  \std{0.2} & 22.5  \std{0.3} & 22.7  \std{0.4} & 22.6  \std{0.3} \\
%         MAML \citep{finn2017model} & 59.3  \std{1.2} & 61.4  \std{1.9} & 61.0  \std{1.8} & 57.3  \std{1.0} & \bf 60.4  \std{0.4} & \bf 63.2  \std{0.7} & \bf 62.6  \std{0.5} & 58.0  \std{0.3} \\
%         ANIL \citep{raghu2019rapid} & 62.4  \std{0.7} & 65.7  \std{0.8} & 64.8  \std{1.3} & 59.5  \std{0.9} & 58.1  \std{0.5} & 61.0  \std{0.8} & 59.7  \std{0.7} & 55.8  \std{0.4} \\
%         BGD \citep{zeno2018task} & 54.8  \std{0.8} & 53.8  \std{1.0} & 54.6  \std{1.9} & 55.3  \std{1.0} & 27.7  \std{0.7} & 27.4  \std{0.7} & 27.7  \std{0.8} & 27.8  \std{0.8} \\
%         MetaCOG \citep{He2019TaskAC} & 55.2  \std{0.7} & 54.1  \std{1.1} & 55.8  \std{1.6} & 55.4  \std{1.0} & 24.5  \std{0.2} & 23.9  \std{0.4} & 24.0  \std{0.3} & 25.1  \std{0.3} \\
%         % MetaBGD \citep{He2019TaskAC} & 42.7  \std{nan} & 42.1  \std{nan} & 43.7  \std{nan} & 42.6  \std{nan} & 46.8  \std{0.8} & 45.8  \std{1.1} & 46.8  \std{1.0} & 47.3  \std{0.9} \\
%         MetaBGD \citep{He2019TaskAC} & 55.9  \std{0.6} & 55.7  \std{0.9} & 54.1  \std{1.4} & 56.8  \std{0.9} & 46.8  \std{0.8} & 45.8  \std{1.1} & 46.8  \std{1.0} & 47.3  \std{0.9} \\
%         \hline 
%         C-MAML & 61.4  \std{0.5} & 59.5  \std{1.4} & 61.2  \std{1.3} & 62.4  \std{0.9} & 53.7  \std{0.3} & 52.0  \std{0.6} & 53.0  \std{0.6} & 54.9  \std{0.5} \\
%         C-MAML + pre. & 59.1  \std{0.9} & 57.4  \std{1.2} & 58.4  \std{1.8} & 60.1  \std{1.2} & 57.8  \std{0.7} & 56.3  \std{0.7} & 57.7  \std{0.9} & 58.6  \std{0.7} \\
%         C-MAML + pre. + \firstFeatureAcron{} & 66.7  \std{0.9} & 65.7  \std{1.7} & 66.2  \std{1.6} & 67.4  \std{0.9} & 59.7  \std{0.3} & 59.1  \std{0.8} & 59.7  \std{0.6} & \bf 59.9  \std{0.4} \\
%         C-MAML + pre. + \firstFeatureAcron{} + \secondFeatureAcron{} & \bf 69.1  \std{0.7} & \bf 68.7  \std{0.9} & \bf 69.3  \std{1.0} &\bf 69.1  \std{1.2} & 53.4  \std{6.4} & 53.5  \std{6.1} & 53.7  \std{6.2} & 53.2  \std{6.6} \\
%         \bottomrule
%     \end{tabular}
%   %}
%   \end{sc}
%   \end{scriptsize}
%   }
%   %\end{tiny}
%   \vspace{-0.12cm}
%   \caption{\textbf{Tiered Imagenet experiment}}
%   \vspace{-0.15cm}
% \label{tab:tiered}
% \end{table*}


% For all benchmarks, we report results on two $\alpha$-locally-stationary environments. The first benchmark's results show online accuracy as function of timesteps in \cref{fig:omniglot} (full results are found in \cref{app:omni}). For Synbols and Tiered-Imagenet, the average accuracies over time are reported in \Cref{tab:synbols,tab:tiered}, respectively. For both regimes, the first column is the average performance over all predictions. The second, third and fourth columns show the performance on the three different settings. The prefix {\small{PRE.}} stands for pretraining. Algorithms perform better in the more locally-stationary regime ($\alpha\!=0\!.98$) because they spend more time in each task before switching.  

% \paragraph{Fast adaptation} We found fast adaptation (or meta-learning) to be the most critical feature for models to perform well in OSAKA, as highlighted by the performance gap between Online ADAM and Continual-MAML (up to +33\% in Synbols $\alpha\!=\!0.90$). This gain comes from two advantages: quickly changing weights after a task/context switch, having slow ($\phi$), and fast ($\theta$) weights, which alleviate catastrophic forgetting.

% \paragraph{Dynamic representations} Next, models need the ability to adapt the embedding space to correctly classify the OoD data. The Synbols font classification task highlights that learning a new mapping from the same inputs to a new output space is challenging when the embedded space is static. Namely, the dynamic representations of Continual-MAML offer a $23.7\%$ and a $28.4\%$ improvement in $\alpha \! = \! 0.98$ compared to MAML and ANIL. This behavior is demonstrated in \cref{fig:omniglot} were these two baselines do not improve their performances over time, which is precisely the goal of CL. Thus, these results demonstrates the inapplicability of current MCL to real scenarios. Although MCL can continually learn new tasks without forgetting, its static embedded space will prevent it from learning tasks lying outside of the pre-training data distribution.


% \paragraph{Computational efficiency} Moreover, adding BGD to slow-down forgetting hinder the acquisition of new knowledge. Removing this feature, e.g. from MetaBGD to Continual-MAML, increases the performance in five out of six experiments and diminishes the computation cost by 80\%. 

% \paragraph{\FirstFeature{}} We now analyse, via ablations, the mechanisms we added to Continual-MAML for further improvements. Modulating the updates improved the performance in Omniglot and Tiered experiments but decreased it in Synbols' (C-MAML {\small{+ PRE.}} vs. C-MAML + {\small{PRE. + UM}}, resulting in an average increase of 1.7\%. In Appendix \ref{app:hparam_analysis}, we show how this mechanism interpolates C-MAML {\small{+ UM}}'s behavior betweeen MAML and C-MAML.  

% \paragraph{\SecondFeature{}} Finally, our \secondFeatureAcron{} enabled by the task boundary detection mechanism helps achieve impressive gains in the locally more stationary regime (+11.5\% and 2.4\% in Synbols and Tiered-ImageNet, respectively). In the other regime ($\alpha=0.90$), the shorter task sequences reduces the room for improvements and the results are inconclusive. We show how task boundary predictions are sensitive to the hyperparameter $\gamma$ in \cref{app:hparam_analysis} in terms of precision and recall.


% % With more frequent switches of distribution ($\alpha=0.90$), methods without meta learning suffered from more performance degradation than in the previous setting ($\alpha=0.98$). In fact, in this setting, multiple models collapsed to a random predictor (Online ADAM, Fine Tuning, BGD, and MetaCOG). 
% % On the other hand, most meta-learning methods suffered from smaller degradation in performance, validating our hypothesis that fast adaptation is a crucial feature for handling rapidly changing data distributions. 

% % When focusing on each particular benchmark, pre-training did not improve Continual-MAML for Omniglot/MNIST/FashionMNIST, as the datasets could be learned rapidly. In the synbols benchmark, the font classification task highlights that learning a new mapping from the same inputs to a new output space is challenging when the embedded space is static. Comparing MAML and ANIL with Continual-MAML + pre-train, we observe that dynamic representations almost doubled the accuracy. In the Tiered-ImageNet benchmark, all tasks are more similar to each other than in Omniglot/MNIST/FashionMNIST or synbols. This setup is more similar to the setups used in \citet{He2019TaskAC, raghu2019rapid, finn2017model}. Thus, for $\alpha \! = \! 0.9$, we found that ANIL was better suited for this task overall, although Continual-MAML was able to yield better performance in the OoD case.



% %--------------------------------------------- CONCLUSION --------------------------------------------------%
% %-----------------------------------------------------------------------------------------------------------%
% \vspace{-\rmSectionSpace}
% \section{Conclusions}
% \label{sec:conclusions}
% \vspace{-\rmSectionSpace}


% We propose \newacron~a new approach to continual learning that focuses on online adaptation, faster remembering and is aligned to real-life applications. This framework is task agnostic, allows context-conditioned targets and task revisiting. Furthermore, it allows pre-training, and introduces OoD tasks at continual-learning time. 
% We show that the proposed setting is challenging for current methods that were not designed for \newacron{}. We introduce Continual-MAML, an initial baseline that addresses the challenges of \newacron{} and we empirically demonstrate its effectiveness.

% % We introduced \newacron, a new CL approach that focuses on online adaptation, fast remembering, and is better aligned with real-life applications. We have shown that the proposed setting is challenging for previous continual learning algorithms and we have proposed Continual-MAML as a new baseline to cope with the challenges introduced by our setting.


% % We propose \newacron~a new approach to continual learning that focuses on online adaptation and fast remembering. This framework is task agnostic, allows pre-training, and introduces OoD tasks at continual-learning time. Furthermore, tasks can be revisited, and different levels of non-stationarity can be tested. We argue that \newacron is better aligned with real-life applications of continual learning. 

% % We show that the proposed setting is challenging for current methods in the literature that were designed for other scenarios. We introduce Continual-MAML, an initial baseline that addresses the challenges of \newacron. Continual-MAML pre-trains a representation that adapts fast to new tasks at continual-learning time. In order to cope with the challenges of \newacron, Continual-MAML detects sudden shifts of the task distribution to incorporate new knowledge to the pre-trained representation. In extensive experiments on Omniglot, MNIST, FashionMNIST, tiered-ImageNet, and synbols we show that Continual-MAML is better suited to \newacron than standard continual learning and meta learning methods, as well as meta-continual learning and continual-meta learning.





% % \newpage
% %-------------------------------------------- BROADER ------------------------------------------------------%
% %-----------------------------------------------------------------------------------------------------------%
% \section*{Broader Impact}

% %The goal of continual learning is to allow 
% %predictive systems to autonomously continue to improve their performance and/or %to accumulate knowledge online. In doing so, autonomous systems cannot forget %their previously acquired knowledge, including values learned before deployment. 
% Our work proposes a more-realistic (synthetic) continual-learning environment. This research could help accelerate the deployment of CL algorithms into applications such as autonomous driving, recommendation systems, information extraction, anomaly detection, and others. A domain often associated with continual learning is health care. %Continual learning through its ability to retain previous knowledge is seen as advantageous in settings where training data cannot be kept indefinitely and, for example, in settings where hospital data could be used to contribute to a population-level model, but may not ``leave'' the hospital premises.
% In health care, patient data is (usually) very sensitive, CL algorithms can be the solution to accumulating knowledge from different hospitals: they can be trained continually across hospitals without the data ever leaving the premise.  


% \textbf{Possible negative impacts:} 
% %As we slowly make our simulated environments more realistic and close the gap between research and application, product teams could be tempted to deploy a CL algorithm in production ahead of time. 
% Our framework enables previous tasks to be forgotten at different rates. If data is patient-level data and different tasks relate to different subset of patients, then it means that the system's performance on past patients could vary. 
% %This could lead to unintended consequences that could be harmful in health care. With a fixed compute and memory budget, it is impossible for an algorithm to accumulate all incoming knowledge without forgetting any. 
% A diagnostic system, for example, could forget how to properly diagnose a patient from a previous population whilst learning about a new one. Further research, possibly at the intersection of continual learning and fairness, is needed before the safe deployment of these algorithms. %We might possibly need guarantees before doing so. 

% \textbf{Possible positive impacts:} 
% The aforementioned negative impact may also be its greatest asset for having a positive impact. 
% Returning to our example, practitioners could understand to what extent a diagnostic system  forgets previous diagnostics. They could then use and develop OSAKA to calibrate their algorithms to match their desiderata (e.g., by choosing when the negative consequence of forgetting may outweight the benefits of additional training data).
% %Enabled by OSAKA, researchers and product teams will have a much better understanding of their algorithms behavior when deployed in real scenarios. OSAKA analyzes algorithms’ ability to handle new data distributions, w.r.t. to the data distribution the model was pre-trained on. It can thus prevent unintended surprises the algorithms could have ahead of time. 


% %Moreover, testing the learning algorithms at multiple levels of non-stationarity, removing the task boundary assumption (task agnostic) and experimenting with stochastic context shifts further removes uncertainty about the behavior of the autonomous agent at deployment time. We thus hope that OSAKA accelerates the safe deployment of CL algorithms. %For health care, as patient data can often not be made public, CL algorithms can be the solution to accumulating knowledge from different hospitals: they can be trained continually across hospitals without the data ever leaving the premise.  




% % \textbf{Limits:} Most of the research in CL is targeted towards class- or task-incremental learning \cite{Goodfellow13, kirkpatrick2017overcoming, rebuffi2017icarl, lopez2017gradient, shin2017continual}. While it is necessary to study these scenarios, they are not realistic enough to gain knowledge on how algorithms will behave once deployed in real-life with the capability to further learn. We provide arguments for this claim throughout the manuscript. We list the desiderata of a realistic evaluation framework in Section 2.3 and we propose OSAKA to address them. 


% % For example, for safety reasons an autonomous vehicle cannot forget previously learned edge cases whilst learning new ones. In another case, by knowledge retention across datasets, CL can enable a diagnostic system to learn about new populations from different hospitals in different countries without the need for client data to ever leave their premise. In other words, it enables a workaround of privacy issues. Further, in this particular example, it is of the utmost importance that a model does not forget how to properly diagnose a previous patient. 


% % \textbf{Impact of research:} We propose a CL setting named Online faSt Adaptation and Knowledge Accumulation (OSAKA). OSAKA simulates a (synthetic) environment where:
% % (1) tasks shifts are sampled stochastically,
% % (2) the task boundaries are unknown (task-agnostic setting), 
% % (3) the target distribution is context-dependent, 
% % (4) multiple levels of non-stationarity are used, 
% % (5) tasks can be revisited. 
% % Furthermore, our evaluation of CL performance is different from the one commonly used in CL.
% % OSAKA brings CL research closer to real-life applications and thus enables researchers to develop novel algorithm that are more aligned with their downstream use cases. Furthermore, it allows product teams to learn about their algorithms' behavior at deployment time before they do deploy them.   



% %% system forgets crucial information (risk to safety, risk to economy, risk to equality, etc)
% %% What is the worst way someone could use your research finding, given no resource constraints?
% %% Who might want to use your research maliciously? Do they have the right resources? Consider computation capabilities, finances, influence, technical ability, domain expertise, access to data. How can the research be made more robust against these actors and their usage?
% %% How could your system be modified to cause intentional or unintentional harm? What are the computation costs of each modification?



% % Finally, we can hope that CL, through its knowledge retention capabilities, will further enable a transfer of knowledge from the companies with enormous amount of private data to smaller ones. This is currently achieved through the open-sourcing of pre-trained models but could be enhanced by CL if said models have the ability to further learn without forgetting.   







% % As machine learning progresses, autonomous systems are are quickly becoming omnipresent in our lives. For a learning system to \textit{autonomously} continue improving its performance or accumulating knowledge once deployed, continual learning (CL) algorithms are essential. It is important that the systems do not forget their previously acquired knowledge, e.g., for safety reasons, an autonomous vehicle shouldn't forget previously learned edge cases whilst learning new ones. Moreover, it is of the utmost importance that these autonomous agents do not forget the values that we teach them before deployment. Finally, CL can have a great positive impact in medicine when privacy puts burden on patients' data. E.g., CL can enable autonomous diagnostic system to learn new populations from different hospitals in different countries without patients' data ever leaving the premise by enabling the model to learn without forgetting the previous populations' diagnostics.


% % Most of the research in CL is targeted towards class- or task-incremental learning \citep{Goodfellow13,kirkpatrick2017overcoming,lopez2017gradient,Shin17,rebuffi2017icarl}. While it is necessary to study these scenarios, they are not realistic enough to gain knowledge on how algorithms will behave once deployed in real-life with the capability to further learn. We provide arguments for this claim throughout the manuscript. We list the desiderata of a realistic evaluation framework in \Cref{ssec:env} and we propose \newacron{} to address them.

% % By analyzing algorithms' ability to handle new data distributions, w.r.t to what the data distribution the model was trained on, we believe that OSAKA brings us one step closer to the safe deployment of continually learning agents. Moreover, testing the learning algorithms at multiple levels of  non-stationarity, remove the task boundary assumption (task agnostic) and focusing on online performance of the agent (instead of final performance) further removes uncertainty about the behavior of the autonomous agent at deployment time.


% % \mytodo{polish}
% % Most of the research in continual learning (CL) is targeted towards class- or task-incremental learning \cite{}. While it is necessary to study these scenarios, they are not realistic because they either require an oracle indicating the current task, or they assume that everything can be learned during training time \cite{martha white}. As a result, it is unlikely that task or class incremental learning produce an impact in our societies.
% % In contrast, in this work we propose that CL should be evaluated in a more dynamic scenario (OSAKA). In OSAKA, the agent encounters new data distributions and has to cope with them. This is more realistic than previous scenarios, since it allows for an agent to be given certain abilities at training time, but it has to adapt to new unexpected situations when deployed. We believe that making progress or solving this new scenario will directly translate into better agents that will have broader impact on the real world.


% \begin{ack}

% Grace,

% Use unnumbered first level headings for the acknowledgments. All acknowledgments
% go at the end of the paper before the list of references. Moreover, you are required to declare 
% funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work). 
% More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2020/PaperInformation/FundingDisclosure}.


% Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
% \end{ack}


% %-------------------------------------------- BILBIO -------------------------------------------------------%
% %-----------------------------------------------------------------------------------------------------------%

% % \bibliographystyle{plain}
% \bibliographystyle{plainnat}
% % \bibliographystyle{apalike}
% \bibliography{ref}

% \newpage
% %-------------------------------------------- APPENDIX ------------------------------------------------------%
% %-----------------------------------------------------------------------------------------------------------%
% \input{supplementary}




% \end{document}

==> resubmission.tex <==
We previously submitted this paper to ICML 2020.

Review Scores:

Reviewer 1: Very good paper, I would like to see it accepted.
Reviewer 2: Borderline paper, but the flaws may outweigh the merits. See (1) below.
Reviewer 3: Borderline paper, but the flaws may outweigh the merits. See (2,3) below.


Meta-Review:

+ well written, clear paper.
+ interesting, challenging, and well-justified setting.

- (1) the proposed OSAKA framework is very similar to the recently proposed MOCA framework. This reduces the significance of the paper.
- (2) inadequate study of algorithm hyper-parameters
- (3) not enough ablation experiments to understand how the proposed algorithm really works and where does the performance comes from.


Following the initial feedback, here are the main updates with respect to our original submission:


With respect to (1), MOCA's framework and OSAKA share some commonalities but are fundamentally different. We did reference MOCA in the original submission, but we had not discussed it in-depth because of that. We since added a paragraph in the related works (Section 5) to highlight their important differences. In addition, we added a longer discussion to contrast both papers in Appendix B.2. In short, the MOCA paper's primary contribution is an algorithm (MOCA) and not the proposed testing framework. They do not expose the problems of previous evaluation settings and accordingly propose improvements. On the contrary, we aim at pushing continual learning beyond its current limits. We strongly believe that both papers can exist and that neither reduces the significance of the other.


With respect to (2), we found Reviewer 3's comment particularly helpful in improving our work. We now provide a hyper-parameter sensitivity analysis that shows how robust our proposed baseline (Continual-MAML) is in Appendix C.3. We provided this analysis in our rebuttal and we believe that this caused Reviewer 3 to raise his final score. We also added another hyper-parameter sensitivity analysis for the boundary-detection task, again in Appendix C.3. In this ablation, we focus on a relevant metric to our work, i.e., precision and recall.

With respect to (3), to be clear, we had already reported an ablation of all mechanisms in the previous version of the paper. As an improvement, we now provide an analysis of the performance of the different methodologies w.r.t. time in Figure 2. This analysis provides a more complete picture that explains where and why our proposed baseline (Continual-MAML) better models the challenges introduced by OSAKA. 

In addition to the above changes, we also updated the manuscript given other suggestions from reviewers, colleagues, and ourselves. In particular, we highlight the following changes: 

(i) we standardized the experimental approach followed in the three proposed benchmarks w.r.t. to hyper-parameter ranges (e.g., timesteps and tasks-sampling probabilities),  

(ii) We reran the hyper-parameter search using a larger hyper-parameter domain and increased the number of trials.

(iii) We increased the number of random seeds in experiments from 5 to 20 to obtain more significant test results.

(iv) We added an Algorithmic view of OSAKA (Algorithm 1).

Finally, we added a new feature to Continual-MAML, named the Prolonged adaptation phase (PAP), which further increases the performance of Continual-MAML compared to other methods and also provides further justification for a hyper-parameter we introduced (gamma, see Section 4 and Algo 2). 


